dQwen3.5: Hybrid-Attention Diffusion Language Models

Adapting a pretrained autoregressive (AR) model is a cost-efficient route to a diffusion language model (DLM). While nearly all such adaptations start from a full-attention transformer, AR modeling has shifted toward hybrid architectures that interleave attention and RNN layers. This creates an obstacle for adaptation: unlike attention, RNNs are structurally causal and nontrivial to bidirectionalize. Despite this mismatch, we investigate whether such backbones can become effective DLMs by adapting Qwen3.5 at 0.8B, 2B, 4B, and 9B scales, yielding the dQwen3.5 family. We find that hybrid backbones can be efficient starting points for adaptation: against a full-attention control, the hybrid reaches a given training loss in about half the tokens. Across scales, dQwen3.5 resembles full-attention DLMs in any-order decoding behavior and performs strongly under parallel decoding.

==> _old/introduction_v1.tex <==
\section{Introduction}
\label{sec:intro}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Diffusion language models (DLMs) generate text by iteratively unmasking positions
rather than emitting tokens strictly left to right, which enables parallel and
any-order decoding, and recent releases are increasingly competitive with
autoregressive (AR) models \citep{nie2025large,ye2025dream}. Training a DLM from scratch is
expensive, however, since reaching parity with a similarly sized AR model can require
an order of magnitude more tokens \citep{nie2024scaling}. AR-to-DLM adaptation sidesteps
this cost: one initializes from a pretrained AR model, makes its causal attention
layers bidirectional, and continues training, yielding a well-performing DLM at a fraction
of the from-scratch budget \citep{cheng2025sdar,gong2025diffullama,ye2025dream}. Nearly every such
adaptation to date has started from a full-attention transformer, whose layers are all
attention. AR modeling has meanwhile moved toward hybrid backbones that interleave
attention with recurrent (RNN) layers \citep{lieber2024jamba,minimax2025minimax01,qwen2026qwen35}, and this
raises a basic question: can a hybrid backbone be adapted into a diffusion model at all?
Unlike attention, whose causal mask can simply be removed, an RNN layer accumulates its
state strictly left to right and cannot be bidirectionalized, so at most the attention
layers can be made to see future context while the recurrent layers stay causal. We
adapt the Qwen3.5 family at 0.8B, 2B, 4B, and 9B into hybrid-attention DLMs, which we
call dQwen3.5, alongside a full-attention control (Qwen3-1.7B) of matched trunk size
trained under the same protocol, and ask whether the result still behaves like a diffusion
model and how it holds up as we scale.


At first glance a hybrid backbone looks poorly matched to any-order generation, since
its recurrent layers remain causal after adaptation. We argue that this causal structure
is far less of an obstacle than it appears, because natural language is itself strongly
left to right: the information needed to predict a token is concentrated in its prefix
\citep{khandelwal2018sharp,oconnor2021what,sun2021do}, which is precisely the bias a causal
recurrent layer encodes. DLMs already reveal this same bias in their own behavior,
decoding in AR-like order whenever the order is left unconstrained, even for models such
as LLaDA that were trained from scratch \citep{gong2026diffucoder}. The recurrent layers therefore
supply a prior the data already prefers, while bidirectionalizing only the attention
layers gives every position the access to future context that the denoising objective
requires. Seen this way, the causal recurrent layers and the bidirectional attention
layers are complementary rather than contradictory, and a hybrid backbone is a
principled and not merely a convenient starting point for a DLM.%


This intuition is borne out by how the adapted models actually decode. On HumanEval we
record, for every position, the step at which it is unmasked, and summarize each
trajectory by its local and global AR-ness, defined as the fraction of adjacent position
pairs, and of all position pairs, that are decoded in left-to-right order; a purely
random decoder scores $0.5$ and a strict AR decoder scores $1.0$. Across all four scales 
\sanjay{put summary table across scales in  intro and refer to details in the appropriate tables and sections later},
dQwen3.5 decodes adjacent positions left to right about $64\%$ of the time, which is well
within the $58$ to $66\%$ band spanned by full-attention DLMs such as LLaDA, Dream,
Dream-Coder, and CoDA, while globally every model, ours included, is strongly AR-like,
ranging from roughly $0.88$ to $0.97$. The hybrid thus carries the same statistical
signature as full-attention DLMs: its causal recurrent layers neither force it into rigid
left-to-right generation nor suppress the any-order decoding that separates diffusion from
AR models.%

Matching the decoding behavior of a DLM is valuable only if the resulting models are also
performant, and remain so with scale.
Against the full-attention control trained on identical data under an identical protocol,
the hybrid reaches any given training loss in roughly half the tokens. After only 50B
adaptation tokens, well below the 200B to 2.3T spent by open DLMs of comparable size,
dQwen3.5 is already competitive with them: at the 1.4B trunk scale it leads CoDA on every
benchmark but one, and at the 6.5 to 7B scale it leads on knowledge and on both HumanEval
variants against Dream and LLaDA, while under parallel decoding the 9B model traces a
competitive accuracy and compute frontier at 100B tokens. Because the four sizes share one
architecture, one protocol, and one data mixture, dQwen3.5 is not four unrelated checkpoints
but a single family spanning more than an order of magnitude in scale. Together with the
matched full-attention control and the released intermediate checkpoints and training
telemetry, this is what makes the family useful: it lets others study how hybrid AR-to-DLM
adaptation behaves as a function of scale, holding everything but size fixed. \sanjay{This para requires the most work to sharpen the benefits of this approach.}


 
We release the dQwen3.5 family at 0.8B, 2B, 4B, and 9B, the full-attention control, and
their intermediate checkpoints and training telemetry at
\url{huggingface.co/UT-IFML}, and document the recipe in Section~\ref{sec:recipe}.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textbf{PREVIOUS INTRO START HERE.}


Diffusion language models (DLMs) enable parallelized, any-order token generation, and recent advances are increasingly competitive with autoregressive (AR) models \citep{nie2025large, ye2025dream}.
However, training from scratch remains a costly endeavor, as DLMs typically require an order of magnitude more tokens to reach parity with similarly sized AR models \citep{nie2024scaling}.
\emph{AR-to-DLM adaptation} has thus emerged as a cost-effective alternative: by initializing from an AR model's weights and making each causal attention layer bidirectional, it becomes possible to train a performant DLM at a fraction of the cost \citep{gong2025diffullama, ye2025dream, cheng2025sdar}.


To date, nearly all such adaptations have started from a standard full-attention transformer, which consists exclusively of causal attention layers.
AR modeling has meanwhile shifted toward \emph{hybrid-attention models} that mix attention and RNN layers~\citep{qwen2026qwen35, lieber2024jamba, minimax2025minimax01}.
However, RNN layers are causal by construction and impractical to bidirectionalize.
In principle, bidirectionalizing only the attention layers gives each position access to future context, but it remains unclear whether this is enough for effective parallel and any-order decoding.

% In principle, while bidirectionalizing only the attention layers gives each position access to future context, it remains unclear whether this suffices for effective parallel and any-order decoding.

% While they have shown strong performance in language modeling, RNN layers are causal by construction and impractical to bidirectionalize.

% While they have shown strong performance in language modeling, it is unclear how well hybrid-attention models might perform for diffusion, as the RNN layers are causal by construction and impractical to bidirectionalize.
% In principle, while bidirectionalizing only the attention layers gives each position access to future context, it remains unclear whether this limited bidirectionality is sufficient for effective parallel and any-order decoding.


% This raises an unconventional design question: can bidirectionalizing only the attention layers preserve the hybrid backbone's capabilities while still enabling parallel, any-order decoding?

% While bidirectionalizing only the attention layers in principle allows each position to receive non-causal information, it does raise a practical question: is this enough to enable effective parallel, any-order decoding?

% This raises an unconventional design question: can bidirectionalizing only the attention minority preserve the strengths of a hybrid backbone while still enabling parallel, any-order decoding?

% This thus presents an unconventional design choice: can we retain the benefits of a hybrid backbone while achieving the parallelization and any-order decoding of a DLM?

% Hybrid backbones therefore present an unexplored design point for diffusion: can a model whose recurrent majority remains causal still support effective parallel, any-order generation?


% While hybrid models have shown strong performance in language modeling

% as the RNN layers are causal by construction

% Notably, an RNN layer is causal by construction, meaning that the architecture still retains a causal bias even if the attention layers are made causal.
% Still, the effectiveness of hybrid models in language modeling makes them a promising candidate for AR-to-DLM adaptation.

% meaning that even if the attention layers are made bidirectional, the architecture still carries a causal bias.

% An RNN layer, however, is causal by construction, so the remaining attention layers carry the bulk of the bidirectionality.
% What that structural bias costs a diffusion model is what we set out to measure.


To investigate the potential of hybrid attention diffusion language models, we perform AR-to-DLM adaptation on the Qwen3.5 model family at four different sizes (0.8B, 2B, 4B, 9B).
Specifically, we bidirectionalize only the causal attention layers, and then perform standard adaptation pretraining.
To better control for architecture, we also adapt a full-attention model, namely Qwen3-1.7B \citep{yang2025qwen3}, which has a similar ``trunk'' (non-embedding, non-head parameters) size to the hybrid Qwen3.5-2B. \sanjay{I dont understand - are you creating a new arch in some way? Is this an ablation study?}

\sanjay{Why is a hybdrid arch qualitatively a reasonable approach? Why is it quantitatively a reasonable approach? How does this scale?}




We further perform extensive evaluations with other open-weight DLMs of various sizes.
Our contributions are as follows.


% In conjunction with other open-weight DLMs such as LLaDA

% we additionally adapt a similarly sized full-attention model


% the Qwen3.5 family at four sizes (0.8B, 2B, 4B, 9B) on approximately 100B tokens.
% The adaptation makes the causal attention bidirectional and leaves the RNN layers structurally unchanged.
% To isolate the role of the architecture, we adapt Qwen3-1.7B \citep{yang2025qwen3}, a similarly sized full-attention model, under the identical recipe as a control.
% We summarize our contributions below.

\paragraph{Findings.}
Against a full-attention control trained on the same data under the same recipe, the hybrid reaches a given training loss with roughly half as many tokens.
After only 50B adaptation tokens, the family is already competitive with open DLMs trained on several times that budget; at 100B, the 9B model traces a competitive accuracy--compute frontier under parallel decoding.
Hybrid trajectories also resemble those of other DLMs: in full-canvas mode at one token per step, adjacent positions are decoded in left-to-right order only $\approx$64\% of the time, compared to 58--66\% for all other DLMs, 50\% for random, and 100\% for AR.

% Hybrid trajectories also resemble that of other DLMs: in full-canvas mode at single-steps, all models decode adjacent positions in left-to-right order only $\approx 63\%$ of the time, compared with 50\% for random and 100\% for AR.


% \paragraph{Findings.}
% Against a full-attention control trained on the same data under the same recipe, the hybrid reaches a given training loss at about half the tokens.
% Hybrid-attention DLMs attain strong single-token decode capabilities at only 50B tokens, and at 100B tokens exhibit parallel decoding performance competitive with other DLMs trained on several times that budget.

% On ordering: 

% Locally, the hybrid's confidence-based decode order matches other DLMs: for all models, adjacent positions are committed left-to-right only 61–66\% of the time, versus 50\% for random order and 100\% for AR decoding.


% However, adapted hybrid-attention DLMs are slightly more AR-like than their full-attention counterparts.
% Downstream results also depend on the AR model we start from and on the quality of the adaptation mixture, not on the backbone alone.


% Hybrid backbones reach any given training loss in about half the tokens the full-attention control needs.
% Adaptation is fast in absolute terms too: at 50B tokens the family is already competitive with open DLMs trained on far more.
% The two properties that separate a DLM from an AR model survive the causal bias: every diffusion model we study decodes in parallel and in any order, and \dqfam{}-9B is indistinguishable from the open DLMs in the order it commits neighboring positions.
% It is a competitive parallel decoder, holding code accuracy as the step budget shrinks (\cref{sec:eval-hybrid}).


\paragraph{Evaluation.}
We compare the hybrid-attention DLMs against the full-attention control and open-weight models like LLaDA, Dream, and Dream-Coder.
We report detailed results of various decoding strategies on standard language, coding, and math benchmarks.




\paragraph{Release.}
We release a family of hybrid-attention DLMs, \dqfam{}, at 0.8B, 2B, 4B, and 9B scales, together with the full-attention control.
We also release their intermediate checkpoints and training telemetry, and document the recipe in \cref{app:training}.

% We release the four adapted models, the full-attention control, their intermediate checkpoints, the detailed training recipe, and the full training telemetry.


==> figures/decode-he60.tex <==
\begin{figure}[p]
\centering
\fitwidth{\includegraphics{figures/raw/decode_he60.pdf}}
\caption{\textbf{Decode order on \texttt{HumanEval/60}.}
Each dot marks when and where a position was unmasked, as in~\cref{fig:decode-he27}.}
\label{fig:decode-he60}
\end{figure}


==> figures/drafts.tex <==
% Figure drafts -- scratch gallery.
%
% CLEARED 2026-08-27 (2). It held the throughput appendix subsection, now
% shipped as C.8 in contents/appendix.tex with figures/throughput.tex. What
% the gallery settled:
%
%   - FIXED BATCH COLUMNS, NOT AN ENVELOPE. A max-over-batch "largest batch
%     that fits" curve is not supportable: the crossover-refinement lengths
%     (1536, 2560, ...) were run at B=1 only, so a naive max SAWTOOTHS; the
%     batch grid is non-uniform across models (the ~1.4B pair reached B=128,
%     the 6.5-7B models only 32); and peak memory at the largest batch tried
%     is usually 19-66 GB of 96, so the GRID, not the hardware, set that
%     ceiling. Columns at fixed B=2,4,8,16 avoid all three.
%   - COMMON SUPPORT PER PANEL. Comparators were never run past 8192 while
%     dQwen3.5-9B reaches 32768; drawing it alone reads as the others failing
%     at lengths nobody attempted.
%   - TWO ENCODINGS WAS THE ORIGINAL BUG. color=model AND linestyle=batch on
%     converging curves is unreadable; promoting batch to panels fixed it.
%   - CoDA and Dream-Coder-7B are omitted as architecture duplicates of the
%     control and Dream-7B.
%
% ---------------------------------------------------------------------------
% EARLIER USE, CLEARED 2026-08-26. It held the speedup-axis candidates for
% fig:decode-7b. Shipped: combined_fig in scripts/sec4_decode_figs.py now draws
% both rows on a shared log2 speedup axis. What the gallery settled:
%
%   - THE CONVERSION NEEDS A LOG AXIS. speedup = BASE/cost, so log(speedup) =
%     log(BASE) - log(cost): affine, slope -1, so on a log axis it is an exact
%     reflection and curves keep their shape. On a linear axis it is a
%     reciprocal -- budgets 64..1024 are spaced 64/128/256/512 and bunch left,
%     their speedups 16x..1x are spaced 8/4/2/1 and bunch right.
%   - THE TWO ROWS NEEDED DIFFERENT WORK. The fixed row was already log2 and
%     took a tick relabel; the threshold row was LINEAR via fit_cost_axis and
%     had to move to log first.
%   - ROWS STAY SEPARATE (Anton). An overlay draft was rejected: confidence-
%     based decoding is not to be drawn on top of fixed-speed decoding.
%   - fit_cost_axis is now unused by combined_fig but still serves
%     frontier_fig, which stays on measured cost.
%
% HOW TO USE IT AGAIN. Add a \subsection*{} per option, \input this file from
% main.tex AFTER \input{contents/appendix}, and clear it once the choice lands.
% ---------------------------------------------------------------------------


==> figures/training-dynamics.tex <==
\begin{figure}[t]
\centering
\fitwidth{\includegraphics{figures/raw/dynamics_overlay.pdf}}
\caption{\textbf{Training dynamics of the \dqfam{} family.} Training loss (top) and masked-token accuracy (bottom) against content (non-PAD/EOS) tokens, from the end of warmup.
\Cref{fig:telemetry} carries the full schedule and the gradient-norm traces.}
\label{fig:training-dynamics}
\end{figure}

